CXL-Interference: Analysis and Characterization in Modern Computer Systems

Compute Express Link (CXL) is a promising technology that addresses memory and storage challenges. Despite its advantages, CXL faces performance threats from external interference when co-existing with current memory and storage systems. This interference is under-explored in existing research. To address this, we develop CXL-Interplay, systematically characterizing and analyzing interference from memory and storage systems. To the best of our knowledge, we are the first to characterize CXL interference on real CXL hardware. We also provide reverse-reasoning analysis with performance counters and kernel functions. In the end, we propose and evaluate mitigating solutions.

==> 07_related_work.tex <==

\section{Related Works}
\label{sec:related_works}


\textbf{CXL devices and systems:}
Since the introduction of CXL, leading companies has released their FPGA prototypes or ASICs
and built various CXL-based systems to accelerate emerging applications~\cite{park2024lpddr,kwon2023failure,jung2022hello,kwon2023cache,wahlgren2022evaluating,ha2022cms}. Due to CXL's ability to maintain cache coherence across multiple CPUs and accelerators, numerous memory pooling solutions have been proposed~\cite{gouk2022direct,jang2023cxl,li2023pond,wang2024rcmp,wang2022enabling,pinto2020thymesisflow,wang2023cxl,ha2023dynamic}. There are also other researches on CXL systems~\cite{sharma2023introduction,cho2023case,park2022scaling,lee2024improving,wang2024lmb}.
However, the above works are all done on simulators or self-developed hardware and our work targets customer-available CXL devices.
Various page migration strategies are proposed~\cite{lagar2019software,agarwal2017thermostat,lee2023memtis,song2023lightweight,kim2023smt,lee2023t,zhou2024toward,xiang2024matryoshka,maruf2023tpp,zhong2024managing,autonuma} to achieve a memory tiering system for CXL. 
We use AutoNUMA~\cite{autonuma} in the experiment, which is the default config in linux kernel.

\textbf{Profiling the CXL FPGA prototypes and ASICs:}
Sun \textit{et al}.~\cite{sun2023demystifying} evaluated a CXL-ready system and compare the performance of ASIC CXL memory and emulated CXL memory. Tang \textit{et al}.~\cite{tang2024exploring} explored the throughput and latency impacts of ASIC CXL memory on applications in various data-center scenarios. Different from prior studies~\cite{sun2023demystifying,tang2024exploring,liu2024exploringevaluatingrealworldcxl} focusing on CXL devices itself, our work dives into the interplay between CXL devices and other devices including memory and storage.


\textbf{Performance guarantee against noisy neighbors:}
Traditional regulation scenarios considers the interference occurring on DRAM and lots of scheduling strategies~\cite{xiang2019emba,chen2019parties} are proposed to guarantee the performance target of applications. With the deployment of NVM, MT$^2$~\cite{yi2022mt} found bandwidth contention on the shared memory bus of hybrid NVM/DRAM platforms and proposed a memory bandwidth regulation solution. Our work focuses on the interference introduced by the emerging CXL devices.


